CLEVRER: CoLlision Events for Video REpresentation and Reasoning

The ability to reason about temporal and causal events from videos lies at the core of human intelligence. Most video reasoning benchmarks, however, focus on pattern recognition from complex visual and language input, instead of on causal structure. We study the complementary problem, exploring the temporal and causal structures behind videos of objects with simple visual appearance. To this end, we introduce the CoLlision Events for Video REpresentation and Reasoning (CLEVRER), a diagnostic video dataset for systematic evaluation of computational models on a wide range of reasoning tasks. Motivated by the theory of human casual judgment, CLEVRER includes four types of questions: descriptive (e.g., "what color"), explanatory ("what is responsible for"), predictive ("what will happen next"), and counterfactual ("what if"). We evaluate various state-of-the-art models for visual reasoning on our benchmark. While these models thrive on the perception-based task (descriptive), they perform poorly on the causal tasks (explanatory, predictive and counterfactual), suggesting that a principled approach for causal reasoning should incorporate the capability of both perceiving complex visual and language inputs, and understanding the underlying dynamics and causal relations. We also study an oracle model that explicitly combines these components via symbolic representations.

==> table/ablated.tex <==
\begin{table*}[t]
    \setlength{\tabcolsep}{2pt}
	\begin{flushleft}
	\begin{center}
    	\begin{tabular}{lcccccccc}
    	\toprule
    	& \multicolumn{4}{c}{Desc.} & \multicolumn{4}{c}{Expl. (per opt./ per ques.)} \\
        \cmidrule(lr){2-5}\cmidrule(lr){6-9}
        \# Prog. & 500 & 1000 & 2000 & all  & 500 & 1000 & 2000 & all \\
        \midrule
        Ours & \textbf{86.01} & \textbf{88.08} & \textbf{88.23} & \textbf{88.39}  & \textbf{84.04/76.30} & \textbf{87.64/79.60} & \textbf{87.66/79.61} & \textbf{87.72/79.67} \\
        Ours* & 83.81 & 85.79 & 85.93 & 86.10 & 82.35/71.23 & 85.92/74.30 & 85.95/74.32 & 86.00/74.37 \\
        \midrule
        & \multicolumn{4}{c}{Pred. (per opt./ per ques.)} & \multicolumn{4}{c}{Cont. (per opt./ per ques.)} \\
        \cmidrule(lr){2-5}\cmidrule(lr){6-9}
        \# Prog. & 500 & 1000 & 2000 & all  & 500 & 1000 & 2000 & all \\
        \midrule
        Ours & \textbf{82.86/68.70} & \textbf{82.86/68.70} & \textbf{82.86/68.70} & \textbf{82.86/68.70} & \textbf{73.36/41.84} & \textbf{74.05/42.23} & \textbf{74.05/42.23} & \textbf{74.05/42.22} \\
        Ours* & 75.38/54.07 & 75.38/54.07 & 75.38/54.07 & 75.38/54.07   & 75.36/41.56 & 76.10/42.01 & 76.10/42.01 & 76.10/42.01 \\
        \bottomrule
    	\end{tabular}
    \end{center}
	\end{flushleft}

	\caption{Ablation study results. * indicates no event supervision.}

	\label{tab:result}
\end{table*}



==> table/dataset_check.tex <==
\begin{table}[t]
	\begin{center}\small
	\begin{tabular}{lccccccc}
	\toprule
         {Dataset} &  CLEVR~\cite{Johnson2017CLEVR} & TGIF-QA~\cite{jang2017tgif} & COG~\cite{Yang2018dataset} & TGIF-QA~\cite{jang2017tgif} &
         MovieQA~\cite{tapaswi2016movieqa}&MarioQA~\cite{Mun2017MarioQA} & CLEVRER (ours)
 
    \bottomrule
	\end{tabular}
	\end{center}
	\vspace{-10pt}
	\caption{The \data dataset is a video reasoning benchmark created under a fully-controlled environment. The dataset incorporates reasoning tasks from various domains including temporal relation, explanation, prediction and counterfacts. \data also comes with detailed annotations of object motion, event history and question program for model diagnostics. \jw{what about making it single-column.}}
	\vspace{-13pt}
	\label{tab:dataset_comparison}
\end{table}

==> text/acknowledgement.tex <==
\myparagraph{Acknowledgement}
We thank Jiayuan Mao for helpful discussions and suggestions. This work is in part supported by ONR MURI N00014-16-1-2007, the Center for Brain, Minds, and Machines (CBMM, funded by NSF STC award CCF-1231216), and IBM Research.

==> text/experiment.tex <==
%\section{Experiments}


%In this section, we evaluate the performance of our model and various baselines on \data, and include human-study results. For all methods we study, we uniformly sample 1 out of 5 frames from the video and use a pretrained ResNet-50~\citep{He2015Deep} to extract the visual features.

\input{figText/model_result.tex}
\input{table/result.tex}

\section{Descriptive Reasoning}

In this section, we evaluate the performance of our model and various baselines on the descriptive questions in \data. Our dataset has 219,815 open-ended descriptive questions in total, including 109,919 questions for training, 54,958 for validation, and 54,938 for testing. There are five sub-types of descriptive questions: \texttt{exist}, \texttt{count}, \texttt{query\_shape}, \texttt{query\_material}, and \texttt{query\_color}. Each sub-type corresponds to an output module in the question program and has its own answer candidates. Details of these sub-types and the answer space can be found in the supplementary material. % including ``yes"/``no" for \textit{exist} ; seven numbers (``0" through ``6") for \textit{count}; two materials (``rubber", ``metal") for \textit{query\_material}: three shapes (``sphere", ``cylinder", ``cube") for \textit{query\_shape}, and eight colors (``gray", ``red", ``blue", ``green", ``brown", ``cyan", ``purple", ``yellow") for \textit{query\_color}.

\subsection{Baselines}

%We consider several representative approaches for the visual reasoning task as baseline models for comparison. 

\paragraph{Q-type (random).} This baseline randomly chooses an answer from the answer candidates of each question’s sub-type.

\myparagraph{Q-type (frequent).} 
Similar to the ``Q-type mode"~\citep{Johnson2017CLEVR} and ``per Q-type prior"~\citep{Antol2015Vqa}, this baseline picks the most frequent answer from the training set for each question sub-type.

\myparagraph{LSTM.} We feed the learned word embeddings of each word~\citep{mikolov2013distributed} from the question as input to an LSTM. The final LSTM hidden state is passed to a multi-layer perceptron (MLP) to predict a distribution over answers. This baseline uses no video information; therefore it models question-conditional bias.

\myparagraph{CNN+MLP.} The question is encoded by averaging word vectors trained on the Google News corpus~\citep{mikolov2013distributed} in the question, and the video is encoded using average pooling features from a convolutional network (CNN). The question and video features are then concatenated and fed into an MLP to predict a distribution over answers~\citep{zhou2015simple}.

\myparagraph{CNN+LSTM.} Video and questions are encoded using CNN features followed by average pooling over frames and final LSTM hidden states, respectively. These features are concatenated to predict an answer distribution.

\myparagraph{MAC (I).} MAC networks~\citep{Hudson2018Compositional} are one of state-of-the-art attention-based models for compositional visual reasoning on images. In this baseline, we directly apply the MAC model to the middle frame of each video.

\myparagraph{MAC (V).} We add a temporal attention unit across all the video frames to generate a latent encoding for the entire video. We then feed it to the MAC network for our video reasoning tasks.

\myparagraph{IEP-EE.} The IEP~\citep{Johnson2017Inferring} model introduces neural program execution for visual reasoning on images. We apply the same approach for our program-based video reasoning task. We replace the input layer of its neural execution engine by a convolutional LSTM~\citep{xingjian2015convolutional} to encode the entire video. The execution engine assembles a dynamic neural module network based on the input program, which is later applied to the video features to produce an answer distribution. Empirically, we observe that the original IEP model does not perform well on our task. In our experiments, we instead train and evaluate the IEP model with ground-truth programs, \ie, we focus on evaluating its execution engine (EE). 

\myparagraph{Implementation details.} We use a pre-trained ResNet-50~\citep{he2016deep} to extract visual features from frames. We use the 2,048-dimensional pool5 layer as the feature representation for CNN-based approaches, and the 14$\times$14 feature maps for MAC.  %All models are trained till convergence. We tune the hyper-parameters on the validation sets and then apply them to the test set. 
Due to memory constraint, we uniformly sample 25 frames (out of 125) for each video as input. All models are trained on the same training set until convergence, tuned on the validation set, and evaluated on the test set. %The evaluation metric uses one ground-truth answer for each question to compute accuracies.


\subsection{Results}

% \jw{Discuss the results figures. Figure 5}
\gc{This paragraph is very confusing. The fluent should be like this (1) our dataset is less bias, since random prior model not working (2) Language only can not achieve good results since the QA need to understand video (3) Different model are good at different tasks, and our dataset is good to differentiate them. MAC good at logic, model with object-centric representation and high-level attributes can help to improve QA performance. (4) We also find that they are both bad at counterfactual, explanatory, since they does have a model can understand dynamics. (5) so we proposed an oracle model}
\fig{fig:result} shows our model's output and intermediate results on a sample video. Given the input, our frame parser detects and extracts object intrinsic attributes and outputs an abstract representation of the objects. The dynamics predictor detects all events (enter, exit, collision) from the observed video, and performs predictive and counterfactual roll-out to obtain unobserved event traces. The questions are parsed into programs, which are then executed on the event traces and object representation to obtain an answer.

\tbl{tab:result} suggests that \model achieves higher accuracy compared with other baselines. Here, we would like to emphasize that our model relies on extra supervision, including object masks and intrinsic attributes such as colors for training the video parser, ground-truth programs for training the question parser, and collision event annotations for training the dynamics predictor. For descriptive questions, two simple baselines (CNN+LSTM and CNN+MLP) achieve higher performance than the text-based LSTM baseline by 4.4\% and 7.1\%. MAC with composition spatial and temporal attention achieves the highest performance among all baselines. %To be noted, our approach requires stronger supervision ( programs) than MAC networks to train the language parser, which is not required for the MAC networks. 
Another interesting observation is that the performance of image-based and video-based MACs differs significantly (67.2\% \vs 84\%). This demonstrates that spatial-temporal cues are crucial for better performance on \data.

% \myparagraph{Human study.} 
We have also conducted a human study on 2,000 randomly selected questions from the test set. We show each case to three humans and take the majority vote as the answer. Humans achieve an accuracy of 91.3\% on these descriptive questions, outperforming our method and all other baselines.

\section{Causal Reasoning}

We now evaluate the performance of various models on causal reasoning, using the explanatory, predictive, and counterfactual questions of \data. Our dataset includes 118,307 multiple choice questions on these three types. We measure the performance of the multiple choice questions based on two criteria: per-option accuracy and per-question accuracy. Per-option accuracy is defined as the percentage of options that are correctly selected/deselected, which measures a model's performance on the option level. Per-question accuracy is the percentage of questions that are correctly answered (\ie, selecting all and only the correct options). Per-question accuracy  requires a comprehensive understanding of the video and is less sensitive to bias.

% measures the model's performance on single-entry level reasoning tasks while accuracy per question 

%\subsection{Experiment Setups}

\subsection{Baselines}

We adopt similar baselines used in the descriptive questions with minor modifications to adapt to the new question types. For all models, we reformulate the multiple choice questions as selecting yes/no for each option, and set their output to a binary indicator.

% \myparagraph{Q-type (random).} This baseline randomly chooses an answer from the answer candidates for each question’s type.

% \myparagraph{Q-type (frequent).} 
% Similar to the ``Q-type mode" in~\citep{Johnson2017CLEVR} and ``per Q-type prior"~\citep{Antol2015Vqa}, this baseline picks up the most frequent training-set answer for each question’s type.

\myparagraph{Q-type.} The Q-type random baseline randomly sets each choice to be true or false with equal probability. The Q-type frequent baseline always selects the most common yes/no option in the training set within each question type. 

\myparagraph{LSTM \& CNN+LSTM \& MAC (I) \& MAC (V).} For these baselines, we add an extra LSTM to encode the option and then concatenate the option encoding with the question encoding. The rest of the networks remains the same.

\myparagraph{CNN+MLP.} We directly concatenate the features of the question, video, and option and feed them in to an MLP with a binary classifier. The question and option are encoded by averaging word vectors.

% We concatenate question features, video features, and answers choice features are then concatenated and fed into an MLP with a binary classifier. Both the question and answers are encoded by averaging word vectors.

\myparagraph{IEP (V).} For each question-option pair, we join the ground-truth program of the question and of the option head to tail, and feed the full program to the IEP execution engine together with the video features. The execution engine outputs a binary label.

\subsection{Results}

% outputs event traces under different running modes. The observation mode detects all events (enter, exit, collision) that are present in the video; Predictive roll-out outputs all collision events that happen after the video ends

% Our model achieves higher accuracy on all question types compared to other baseline, but also relies on extra overall supervisions, including the object masks and intrinsic attributes for training the video parser, the ground-truth programs for training the question parser, and the collision event annotations for training the dynamics predictor.

\fig{fig:result} shows that our model captures the predictive and counterfactual events and leverages that information to generate the correct answer. \tbl{tab:result} suggests that it outperforms the baselines on all three types of questions. Most baselines achieved a 0\% accuracy on predictive questions. This is because there are relatively fewer predictive questions, compared with questions of other types, and for most predictive questions, only one of the four options is correct. In such case, these baselines simply output `no' for all options. Again, we would like to emphasize that though our model performs well, it requires extra annotations during training. Building model that learn from only videos and question-answer pairs remain a future research direction.

% In our result
% Almost all the baseline models fails on the . We see two main
% explanations for this. First, answering the counterfactual and predictive questions require a dynamic model to for the simulation and inference. Current VQA models can hardly to  scenarios. Second, the visual information for these question are not dominant. The neural networks are vulnerable to overfitting to the bias of questions and answers. For instance, we analyze the results of predictive questions, and find that all the predictions for this question type are the same answer. This is not surprising since we only have less than 1,000 training data in this question type. The network tends to find shortcut to answer the question.

We have also conducted a human study on 200 randomly selected test cases for each question type. We ask each question to three subjects and take their majority vote. Per-option accuracies for the explanatory, predictive, and counterfactual questions are 94.2\%, 92.5\%, and 81.6\%, respectively, and per-question accuracies are 87.1\%, 74.5\%, and 58.1\%. 
  


